Refined Large Deviation Principle for Branching Brownian Motion Conditioned to Have a Low Maximum

Conditioning a branching Brownian motion to have an atypically low maximum leads to a suppression of the branching mechanism. In this note, we consider a branching Brownian motion conditioned to have a maximum below $\sqrt{2}\alpha t$ ($\alpha<1$). We study the precise effects of an early/late first branching time and a low/high first branching location under this condition. We do so by imposing additional constraints on the first branching time and location. We obtain large deviation estimates, as well as the optimal first branching time and location given the additional constraints.

==> Sections/LDP-BBM-def.tex <==
 %xdvi ted:       Wed 11 Oct 2006 13:51:07 CEST
%Last Modified:     Thu 14 Jun 2007 14:35:42 CEST
% Modified by Yanjia, Mon 14 Sep 2020
%<<< Preamble
\usepackage[headinclude,DIV13]{typearea}
\areaset{15.1cm}{25.0cm}
\parskip 0pt plus .5pt
\usepackage{txfonts,amssymb,amsmath,amsthm,bbm,physics}
\usepackage{cases}

\usepackage[latin1] {inputenc}
\usepackage{graphicx, psfrag}
\usepackage{setspace}
\usepackage{xcolor}
%\usepackage{subfigure}
\usepackage{subcaption}
\usepackage{enumerate}

\graphicspath{{Figures/}}

\renewcommand {\familydefault}   {ptm}  

\usepackage{appendix}

\usepackage{hyperref}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}{Condition}
\newtheorem{solution}{Solution}

%%%%% by Yanjia
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Prob}[1]{\mathbb{P}\left(#1\right)}
\newcommand{\E}[1]{\mathbb{E}\left(#1\right)}
\newcommand{\cT}{\mathcal{T}}

\renewcommand{\l}[2]{\ensuremath{I_{#1}\left(#2\right)}}
\renewcommand{\ll}[3]{\ensuremath{I_{#1}\left(#2;\,#3\right)}}

\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}


%%%%%Colours
\definecolor{bbm}{RGB}{51,153,0}
\definecolor{above}{RGB}{128,0,128}
\definecolor{below}{RGB}{102,0,204}
\definecolor{cascade}{RGB}{204,0,0}
\definecolor{iid}{RGB}{153,51,0}
%%%%

\newtheorem{question}{Question}

\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\newtheorem*{hint}{Hints}

\def\paragraph#1{\noindent \textbf{#1}}

\numberwithin{equation}{section}

\def\todo#1{\marginpar{\raggedright\footnotesize #1}}
\def\change#1{{\color{green}\todo{change}#1}}
\def\comment#1{{\color{green}\todo{Comment}#1}}

\def\ppconv{\overset {pp} \to }
\def\weakconv{\overset w\to }

\def\laweq{\overset{\mathrm{law}}=}
\def\lawconv{\xrightarrow[N\to\infty]{\text{law}}}

\def\Max{{\mathrm{max}}}
\def\Min{{\mathrm{min}}}
\def\supp{\mathop{\mathrm{supp}}\nolimits}
\def\Id{\mathrm{Id}}
\def\dist{\mathop{\rm dist}\nolimits}
\def\Var{\mathop{\rm Var}\nolimits}
\def\Cov{\mathop{\rm Cov}\nolimits}
\def\supp{\mathop{\rm supp}\nolimits}
\def\sign{\mathop{\rm sign}\nolimits}
\def\d{\mathrm{d}}
\def\dd{\mathtt{d}}

\def\bbone{\boldsymbol 1 }
\def\rf{\rfloor}

\def\lf{\lfloor}

\def\<{\langle}
\def\>{\rangle}

\def\a{\alpha}
\def\b{\beta}
\def\e{\epsilon}
\def\ve{\varepsilon}
\def\f{\phi}
\def\g{\gamma}
\def\k{\kappa}
%\def\l{\lambda}
\def\r{\rho}
\def\s{\sigma}
\def\t{\tau}
\def\th{\theta}
\def\vt{\vartheta}
\def\vp{\varphi}
\def\z{\zeta}
\def\o{\omega}
\def\D{\Delta}
\def\L{\Lambda}
\def\G{\Gamma}
\def\O{\Omega}
\def\S{\Sigma}
\def\Th{\Theta}
\def\h{\eta}
\def\del{\partial}
\def\R{{\Bbb R}}  
\def\N{{\Bbb N}}  
\def\P{{\Bbb P}}  
\def\Z{{\Bbb Z}}  
\def\Q{{\Bbb Q}}  
\def\C{{\Bbb C}} 
\def\E{{\Bbb E}}  
\def\M{{\Bbb M}}  
\def\U{{\Bbb U}}
\def\Va{{\Bbb V}}  
\def\T{{\Bbb T}}

\let\cal=\mathcal
\def\AA{{\cal A}}
\def\BB{{\cal B}}
\def\CC{{\cal C}}
\def\DD{{\cal D}}
\def\EE{{\cal E}}
\def\FF{{\cal F}}
\def\GG{{\cal G}}
\def\HH{{\cal H}}
\def\II{{\cal I}}
\def\JJ{{\cal J}}
\def\KK{{\cal K}}
\def\LL{{\cal L}}
\def\MM{{\cal M}}
\def\NN{{\cal N}}
\def\OO{{\cal O}}
\def\PP{{\cal P}}
\def\QQ{{\cal Q}}
\def\RR{{\cal R}}
\def\SS{{\cal S}}
\def\TT{{\cal T}}
\def\VV{{\cal V}}
\def\UU{{\cal U}}
\def\VV{{\cal V}}
\def\WW{{\cal W}}
\def\XX{{\cal X}}
\def\YY{{\cal Y}}
\def\ZZ{{\cal Z}}


\def \X {{\Xi}}
\def \G {{\Gamma}}
\def \L {{\Lambda}}
\def \k {{\kappa}}
\def \b {{\beta}}
%\def \e {{\varepsilon}}
\def \s {{\sigma}}
\def \h {{\eta}}
\def \z {{\zeta}}
\def \m {{\mu}}
\def \n {{\nu}}
\def \D {{\Delta}}
\def \t {{\tau}}
\def \th {{\theta}}
\def \T {{\Theta}}
\def \g {{\gamma}}
%\def \l {{\lambda}}
\def \d {{\delta}}
\def \a {{\alpha}}
\def \o {{\omega}}
\def \O {{\Omega}}
\def \th {{\theta}}
\def \n {{\nu}}
\def \x {{\xi}}
\def \del {{\partial}}
\def \f {{\phi}}
\def \vf{{\varphi}}
\def \F {{\Phi}}
\def \r {{\rho}}
\def \c {{\chi}}

\def \ba {\begin{array}}
	\def \ea {\end{array}}


\def\bL{\mathfrak L}

%%%%%%%%%%%%%%%%%%%% Macros %%%%%%%%%%%%%%%%%%%%%%%%%
\def \A {{\mathbb A}}
\def \B {{\mathbb B}}
%\def \D {{\mathbb D}}
\def \X {{\mathbb X}}

\def \fru {{\mathfrak u}}
\def \frf {{\mathfrak f}}
\def \frF {{\mathfrak F}}



\def \cA {{\cal A}}
\def \cB {{\cal B}}
\def \cC {{\cal C}}
\def \cD {{\cal D}}
\def \cE {{\cal E}}
\def \cF {{\cal F}}
\def \cG {{\cal G}}
\def \cH {{\cal H}}
\def \cI {{\cal I}}
\def \cL {{\cal L}}
\def \cM {{\cal M}}
\def \cN {{\cal N}}
\def \cP {{\cal P}}
\def \cQ {{\cal Q}}

\def \cR {{\cal R}}
\def \cS {{\cal S}}
\def \cU {{\cal U}}
\def \cV {{\cal V}}
\def \cW {{\cal W}}
\def \cX {{\cal X}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
%\def\TH(#1){\label{#1}}\def\thv(#1){\ref{#1}}
%\def\Eq(#1){\label{#1}}\def\eqv(#1){(\ref{#1})}
\def\diam{\hbox{\rm diam}}
\def\cov{\hbox{\rm Cov}}
\def\var{\hbox{\rm Var}}
\def\sfrac#1#2{{\textstyle{#1\over #2}}}

\def\bra#1{\langle #1 \rangle}
\def\arcth{\hbox{\rm arcth}}
\def\capa{\hbox{\rm cap}}
\def \1{\mathbbm{1}}
\def\wt {\widetilde}
\def\wh{\widehat}


\def \bz {{\boldsymbol z}}
\def \bx{{\boldsymbol x}}
\def \by{{\boldsymbol y}}
\def \bu {{\boldsymbol u}}
\def \bm{{\boldsymbol m}}
\def \bfe{{\boldsymbol e}}
\def \bv {{\boldsymbol v}}
\def \bw {{\boldsymbol w}}
\def \bI {{\boldsymbol I}}
\def \bC {{\boldsymbol C}}
\def \bA {{\boldsymbol A}}
\def \bB {{\boldsymbol B}}
\def \bG {{\boldsymbol G}}
\def \bU {{\boldsymbol U}}
\def\brho{{\boldsymbol \rho}}
\def\checkv{{\boldsymbol {\check v}}}


%%%%%%%%%%%%%%%%%%%% Macros %%%%%%%%%%%%%%%%%%%%%%%%%
\def\leb{\hbox{\rm Leb}}
\def\PRM{\hbox{\rm PRM}}
\def\asl{\hbox{\rm Asl}}

\def \fru {{\mathfrak u}}
\def \frf {{\mathfrak f}}
\def \frF {{\mathfrak F}}
\def \zet {{\mathfrak z}}


\def \lb {\left(}
\def \rb {\right)}
\def \lbr {\left\{}
\def \rbr {\right\}}
\def \df {\stackrel{\Delta}{=}}
\def \sign{\hbox{\rm sign}}



\def \so {\text{\small{o}}(1)}
\def \po {\text{\small{o}}}

\def\vm{\bm}




\def\ubx{\underline{\bx}}
\def\us{\underline{\s}}

\def\eee{{\mathrm e}}
\def \so {\text{\small{o}}(1)}
\def \po {\text{\small{o}}}

\def\vm{\bm}




\def\ubx{\underline{\bx}}
\def\us{\underline{\s}}

\def\eee{{\mathrm e}}

